Interpretable Deep Feature Propagation for Early Action Recognition

Early action recognition (action prediction) from limited preliminary observations plays a critical role for streaming vision systems that demand real-time inference, as video actions often possess elongated temporal spans which cause undesired latency. In this study, we address action prediction by investigating how action patterns evolve over time in a spatial feature space. There are three key components to our system. First, we work with intermediate-layer ConvNet features, which allow for abstraction from raw data, while retaining spatial layout. Second, instead of propagating features per se, we propagate their residuals across time, which allows for a compact representation that reduces redundancy. Third, we employ a Kalman filter to combat error build-up and unify across prediction start times. Extensive experimental results on multiple benchmarks show that our approach leads to competitive performance in action prediction. Notably, we investigate the learned components of our system to shed light on their otherwise opaque natures in two ways. First, we document that our learned feature propagation module works as a spatial shifting mechanism under convolution to propagate current observations into the future. Thus, it captures flow-based image motion information. Second, the learned Kalman filter adaptively updates prior estimation to aid the sequence learning process.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> paper_components/bit_base_comp.tex <==
\begin{table*}
\centering
\caption{
Compare proposed method with baseline methodology that uses partial video for recognition without propagation. Our method gain large improvements when observation ratio is lower than 0.5 and achieves similar results afterwards.  
}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline

         & 0.1   & 0.2   & 0.3   & 0.4   & 0.5   & 0.6   & 0.7   & 0.8   & 0.9   & 1.0   \\ \hline
BaseLine & 28.12 & 31.25 & 42.19 & 66.41 & 82.03 & 89.06 & 91.04 & 91.41 & 92.97 & 92.97 \\ \hline
RGN-KF   & 35.16 & 46.09 & 67.98 & 75.78 & 82.03 & 88.28 & 92.19 & 88.28 & 92.16 & 92.19 \\ \hline
\end{tabular}
\label{table: bit_base_comp}
\end{table*}

==> paper_components/feature_vis.tex <==
\begin{figure}[bt]
\center
\includegraphics[width=.9\linewidth]{paper_components/visualization_3.pdf}
\caption{
Visualization of Features and Residuals. The example shows a sequence of frames for the action {\em baseball-swing} along the left hand side. Example feature maps extracted at various layers are shown along the upper/bottom row, while their residuals are shown along the middle row.}
\label{fig:fea_vis}
\end{figure}

==> paper_components/jhmdb21_rst_table.tex <==
\begin{table}[]
\small
\centering
\begin{tabular}{l c}
\toprule
Method            & \multicolumn{1}{l}{Accuracy (\%)} \\ 
\midrule
ELSTM \cite{sadegh2017encouraging}             & 55                            \\ 
Within-class Loss \cite{ma2016learning} & 33                            \\ 
DP-SVM \cite{soomro2019online}           & 5                             \\ 
S-SVM \cite{soomro2019online}            & 5                             \\ 
Where/What \cite{soomro2016predicting}        & 10                            \\ 
Context-fusion \cite{jain2016recurrent}    & 28                            \\ 
RBF-RNN \cite{shi2018action}           & 73                            \\ 
RGN-KF \cite{zhao2019}              & 78               \\ 
RGN-KF-2              & \textbf{79}                 \\ 
Baseline              & 74                 \\ 
\bottomrule
\end{tabular}
\label{table:jhmdb}
\caption{Action Prediction Results on JHMDB21. Following the standard protocol, accuracy results are shown only for the case where initial observations are limited to the first 20\% of frames, \ie $g=0.2$.
}
\end{table}

==> paper_components/jhmdb_reco.tex <==
\begin{table}[]
\centering
\caption{
Performance against state-of-the-art results on \textit{JHMDB-21} dataset with full obervations. The temporal reglarization enforced by Kalman Filtering $Update$ contributes to a tigher temporal semantic consistence.
}
\begin{tabular}{|l|l|}
\hline
Method                                      & Accuracy (\%)\\ \hline
PoTion \cite{choutas2018potion}                                     & \textbf{85.5}     \\ \hline
Chaines Mutiple-Stream \cite{zolfaghari2017chained}                     & 76.1     \\ \hline
Non-Linear Temporal Subspace \cite{cherian2018non} & 74.2     \\ \hline
Generalized Rank Pooling \cite{cherian2017generalized}                   & 73.7     \\ \hline
Higher Order Pooling \cite{cherian2017higher}                          & 73.3     \\ \hline
P-CNN \cite{cheron2015p}                                   & 72.2     \\ \hline
Baseline (TSN)                                    & 82.1     \\ \hline
RGN-KF                                      & 83.4     \\ \hline
\end{tabular}
\label{table:jhmdb_top}
\end{table}

==> paper_components/multi_fea_stg_comp.tex <==
%\documentclass[10pt,twocolumn,letterpaper]{article}
%\usepackage{multirow}
%\begin{document}
\begin{table*}[h]
\centering
\begin{tabular}{l c c c c c c c c c}
\toprule
          & \multicolumn{4}{c}{UCF-101} & \multicolumn{4}{c}{BIT}      & JHMDB-21 \\ 
\cmidrule(l){2-10}
\textit{observation ratio}         & 0.1   & 0.2  & 0.3   & 0.8  & 0.1   & 0.2   & 0.3   & 0.8   & 0.2      \\
\midrule
56x56x64  &    83.16   &   85.03    &   87.92    &   92.10   & 33.41 & 46.65 & 67.51 & 84.38 & 75.83    \\ 
28x28x192 &    83.78   &   86.22    &   89.01    &   93.07   & 37.33 & 49.96 & 69.12 &  88.82 & 79.00    \\ 
14x14x576 &    83.29   &   85.46   &    88.19   &   93.06  & 36.62 & 48.70 & 68.19 & 87.50 & 77.63    \\ 
7x7x1024  &    80.51   &    84.94   &    88.17   &    92.77  &  36.12&  49.22 &  67.61 & 87.50 & 77.42    \\ 
\bottomrule
\end{tabular}
\label{table: FeaStg}
\caption{
Prediction Accuracy (\%) at Various Intermediate Feature Stages with \textbf{RGN-KF-2}, Ordered by Decreasing Spatial Receptive Field Size. Observation ratio $g \in \{ 0.1, 0.2, 0.3, 0.8 \}$ for UCF101 and BIT datasets. Set $g = 0.2$ for JHMDB21.
}
\end{table*}
%\end{document}

==> paper_components/multi_fea_stg_comp_-_Copy.tex <==
%\documentclass[10pt,twocolumn,letterpaper]{article}
%\usepackage{multirow}
%\begin{document}
\begin{table*}[h]
\centering
\begin{tabular}{l c c c c c c c c c}
\toprule
          & \multicolumn{4}{c}{UCF-101} & \multicolumn{4}{c}{BIT}      & JHMDB-21 \\ 
\cmidrule(l){2-10}
\textit{observation ratio}         & 0.2   & 0.4  & 0.6   & 0.8  & 0.2   & 0.4   & 0.6   & 0.8   & 0.2      \\
\midrule
56x56x64  &    85.16   &   88.64    &   91.10    &   92.10   & 35.94 & 49.22 & 75.78 & 84.38 & 75.74    \\ 
28x28x192 &    85.16   &   90.78    &   92.03    &   93.19   & 46.09 & 75.78 & 88.28 &  88.82 & 78.30    \\ 
14x14x576 &    85.09   &   90.32   &    92.12   &   93.06  & 40.62 & 76.65 & 85.94 & 87.50 & 77.43    \\ 
7x7x1024  &    84.94   &    90.07   &    91.60   &    92.77  & 42.06 & 75.78 & 87.50 & 87.50 & 77.03    \\ 
\bottomrule
\end{tabular}
\label{table: FeaStg}
\caption{
Prediction Accuracy (\%) at Various Intermediate Feature Stages with \textbf{RGN-KF}, Ordered by Decreasing Spatial Receptive Field Size. Observation ratio $g \in \{ 0.2, 0.4, 0.6, 0.8 \}$ for UCF101 and BIT datasets. Set $g = 0.2$ for JHMDB21.
}
\end{table*}
%\end{document}

==> paper_components/residual_process.tex <==
\begin{figure}[t!]
%paper_graph_v2
%\includegraphics[width=\linewidth]{paper_components/residual_process.pdf}
\includegraphics[width=\linewidth]{paper_components/residual_process_v4.pdf}
\caption{
Residual Based Feature Propagation Process. The proposed approach relies on residual motion between adjacent frames for temporal extrapolation. R Frame (\textcolor{red}{yellow}) represents the very initial reference frame. Residual (\textcolor{blue}{blue}) is the temporal subtraction. P Frame (\textcolor{green}{green}) is the predicted residual that then is used for estimating the real feature from the  Reference Frame. The entire process recursively generates all features.
}\label{fig:teaser}
\end{figure}

==> paper_components/result_graph1.tex <==
\begin{figure*}[bt!]
\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\scalebox{0.3}{\input{paper_components/UCF101_Accuracy.pgf}}
		\caption{UCF-101 dataset}
		\label{fig:1a}
	\end{subfigure}
	\iffalse
	\begin{subfigure}[b]{0.33\textwidth}
		\centering
		\scalebox{0.26}{\includegraphics{./paper_components/JHMDB.pdf}}
		\caption{JHMDB dataset}
		\label{fig:1b}
	\end{subfigure}
	\fi
		\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\scalebox{0.3}{\input{paper_components/BIT_Accuracy.pgf}}
		\caption{BIT dataset}
		\label{fig:1c}
	\end{subfigure}
\caption{
Action Prediction Results on the  UCF101, JHMDB-21 and BIT Datasets at all Observation Ratios $g \in [0.1, 1]$.
}
\label{fig:result}
\end{figure*}

==> paper_components/sparse_feature_check.tex <==
\begin{figure}[h]
\center
\includegraphics[width=1.0\linewidth]{paper_components/sparse_feature_check_v2.pdf}
\caption{
Sparsity Comparison of Features and Residuals. The top row shows frames from a video of a \textit{kicking} action. The bottom row shows sparsity as the ratio of near-zero value points (absolute value $< 0.01$) to total points over time. On average, residual and original feaure points are 65\% and 14\% sparse, resp.
%Ratio of near-zero feature points (absolute value $< 0.01$) to total feature points over time. Residual Feature owns average 65\% sparse points while original feature only possesses average 14\%.  
}
\label{fig:sparse_check}
\end{figure}

==> paper_components/temporal_model.tex <==
\begin{table}[]
\centering
\begin{tabular}{l c }
\toprule
Temporal Propagation Approach & Accuracy (\%) \\ 
\midrule
\small{ConvLSTM(3x3)-128-192-\textbf{Org}}               & \small{71.1}        \\ 
\small{ConvLSTM(3x3)-128-192-\textbf{Org}-\textbf{KF}}               &  \small{73.4}        \\ 
\small{ConvLSTM(3x3)-128-192-\textbf{Org}-\textbf{KF-2}}               &  \small{74.3}        \\ 
\small{ConvLSTM(3x3)-128-192-\textbf{Res}}               &  \small{76.8}        \\ 
\small{ConvLSTM(3x3)-128-192-\textbf{Res}-\textbf{KF}}               &  \small{77.1}        \\  
\small{ConvLSTM(3x3)-128-192-\textbf{Res}-\textbf{KF-2}}               &  \small{77.3}        \\  
\small{RGN-\textbf{Org}}                    & \small{70.9}        \\ 
\small{RGN-\textbf{Org}-\textbf{KF}}                    & \small{74.4}        \\
\small{RGN-\textbf{Org}-\textbf{KF-2}}                    & \small{74.7}        \\  
\small{RGN-\textbf{Res}}                    & \small{77.4}        \\ 
\small{RGN-\textbf{Res}-\textbf{KF}}                    & \small{78.3} \\
\small{RGN-\textbf{Res}-\textbf{KF-2}}                    & \small{\textbf{79.0}}               \\ 
\bottomrule
\end{tabular}
\label{tab:temporal_model}
\caption{
Accuracy results for different temporal propagation approaches on JHMDB21 split 1. \textbf{Org} denotes applying motion kernel transformation on original features, \textbf{Res} denotes residual propagation and \textbf{KF*} denotes inclusion of the Kalman filter. For ConvLSTM, (3x3), 128 \& 192 represent kernel, hidden state \& feature dimension, resp.}
\end{table}
